A Definition of Continual Reinforcement Learning

In a standard view of the reinforcement learning problem, an agent's goal is to efficiently identify a policy that maximizes long-term reward. However, this perspective is based on a restricted view of learning as finding a solution, rather than treating learning as endless adaptation. In contrast, continual reinforcement learning refers to the setting in which the best agents never stop learning. Despite the importance of continual reinforcement learning, the community lacks a simple definition of the problem that highlights its commitments and makes its primary concepts precise and clear. To this end, this paper is dedicated to carefully defining the continual reinforcement learning problem. We formalize the notion of agents that "never stop learning" through a new mathematical language for analyzing and cataloging agents. Using this new language, we define a continual learning agent as one that can be understood as carrying out an implicit search process indefinitely, and continual reinforcement learning as the setting in which the best agents are all continual learning agents. We provide two motivating examples, illustrating that traditional views of multi-task reinforcement learning and continual supervised learning are special cases of our definition. Collectively, these definitions and perspectives formalize many intuitive concepts at the heart of learning, and open new research pathways surrounding continual learning agents.

==> proofs/lemmas/crl_agents_not_all_agents.tex <==
\begin{dproof}[\cref{lem:crl_agents_not_allagents}]
We proceed toward contradiction and suppose that we have an instance of CRL $(\env, \valuef, \agents, \agentsbasis)$ where $\agents=\allagents$. But, by \cref{prop:all_agents_generates_reaches}, we know that all agents will always reach $\agents$, and therefore, every optimal agent $\agent^* \in \agents^*$ satisfies $\agent \alwaysreaches \agents$. This directly violates the definition of CRL, and we conclude. \qedhere
\end{dproof}

==> proofs/lemmas/crl_agents_not_subset_basis.tex <==
\begin{dproof}[\cref{lem:crl_agents_not_subset_basis}]
We proceed toward contradiction and suppose we have a CRL instance $(\env, \valuef, \agents, \agentsbasis$) such that $\agent \subseteq \agentsbasis$. Recall that by \cref{prop:agent_in_set_reaches_set}, we know that any agent $\agent$ in a set $\agents$ also always reaches that set, $\agent \alwaysreaches \agents$. Thus, if $\agents \subseteq \agentsbasis$, we know that every agent $\agent \in \agents$ always reaches the basis, $\agent \alwaysreaches \agentsbasis$.

Since the set of optimal agents,
\[
\agents^* = \argmax_{\agent \in \agents} \valuef(\agent, \env),
\]
is a subset of $\agents$, it follows that every optimal agent $\agent^* \in \agents^*$ also satisfies $\agent^* \alwaysreaches \agentsbasis$. But this directly violates the condition of CRL: recall that the definition of CRL requires that every optimal agent \textit{never reaches} the given basis. We conclude that every tuple $(\env, \valuef, \agents, \agentsbasis)$ where $\agents \subseteq \agentsbasis$ is not an instance of CRL. \qedhere
\end{dproof}

==> proofs/props/always_a_minimal_basis.tex <==
\begin{dproof}[\cref{prop:always_minimal_basis}]
TODO
\end{dproof}

==> proofs/props/complement_generates.tex <==
\begin{dproof}[\cref{prop:complement_generates}]
TODO
\end{dproof}

==> proofs/props/conv_implies_cinfty_bounded.tex <==
\begin{dproof}[\cref{prop:conv_implies_cinfty_bounded}]
\dnote{todo}
Recall that the definition of an agent converging to a bounded agent basis $\boundagentsbasis$ asserts that $\agent \alwaysreach \boundagentsbasis$. Therefore, expanding the definition of $\alwaysreach$, we find
\[
\forall_{h \in \rhistories} \exists_{t \in \mathbb{N}_0} \forall_{h^\circ \in \rsuffhistories^{t:\infty}} \exists_{\agentbasis \in \boundagentsbasis} \forall_{h' \in \rsuffhistories}\ \agent(hh^\circ h') = \agentbasis(hh^\circ h').
\]
Further, when $c_\infty(\agent,\env) \leq n$, we know that
\[

\]
\end{dproof}

==> proofs/props/crl_agents_is_allagents.tex <==
\begin{dproof}[\cref{prop:crl_agents_is_allagents}]
TODO
\end{dproof}

==> proofs/props/crl_agents_not_minimal.tex <==
\begin{dproof}[\cref{prop:crl_agents_not_minimal}]
We first show that $\agents$ cannot be minimal. To do so, we consider the cases where the rank of $\agents$ is finite and infinite separately.\\

% Finite rank case.
\textit{(Finite Rank $\agents$.)} \\

If $\rank(\agents)$ is finite and minimal, then it follows immediately that there is no agent set of smaller rank that generates $\agents$. By consequence, since $\agentsbasis \subset \agents$ and $\agentsbasis \generates \agents$, we conclude that $\agents$ cannot be minimal. \checkmark \\


% Infinite rank case.
\textit{(Infinite Rank $\agents$.)} \\

If $\rank(\agents)$ is infinite and minimal, then there is no proper subset of $\agents$ that uniformly generates $\agents$ by definition. By consequence, since $\agentsbasis \subset \agents$ and $\agentsbasis \generates \agents$, we conclude that $\agents$ cannot be minimal. \checkmark \\
% Need to connect uniformly generates to env-generates?

This completes the argument of both cases, and we conclude that for any instance of CRL, $\agents$ is not minimal.

We next show that $\agents$ cannot be the set of all agents. To do so, we proceed toward contradiction and suppose that we have an instance of CRL $(\env, \valuef, \agents, \agentsbasis)$ where $\agents=\allagents$. But, by \cref{prop:all_agents_generates_reaches}, we know that all agents with always reach $\agents$, and therefore, every optimal agent $\agent^* \in \agents^*$ satisfies $\agent \alwaysreaches \agents$. This directly violates the definition of CRL, and we conclude. \checkmark

This concludes the argument of both properties. \qedhere
\end{dproof}

==> proofs/props/crl_agents_not_subset_basis.tex <==
\begin{dproof}[\cref{prop:crl_agents_not_subset_basis}]
Recall that by \cref{prop:agent_in_set_reaches_set}, we know that any agent $\agent$ in a set $\agents$ also always reaches that set, $\agent \alwaysreaches \agents$. Thus, if $\agents \subseteq \agentsbasis$, we know that every agent $\agent \in \agents$ always reaches the basis, $\agent \alwaysreaches \agentsbasis$.

Since the set of optimal agents,
\[
\agents^* = \argmax_{\agent \in \agents} \valuef(\agent, \env),
\]
is a subset of $\agents$, it follows that every optimal agent $\agent^* \in \agents^*$ also satisfies $\agent^* \alwaysreaches \agentsbasis$. But this directly violates the condition of CRL: recall that the definition of CRL requires that every optimal agent \textit{never reaches} the given basis. We conclude that every tuple $(\env, \valuef, \agents, \agentsbasis)$ where $\agents \subseteq \agentsbasis$ is not an instance of CRL. \qedhere
\end{dproof}

==> proofs/props/eventually_xor_never_reaches.tex <==
\begin{dproof}[\cref{prop:eventually_xor_never_reaches}]
The proof is again relatively straightforward, as the two statements are simply logical negations of one another.

That is, recall the definition of $\agent \reaches \agentsbasis$ for a fixed but arbitrary $(\agent, \agentsbasis)$ pair:
\begin{equation}
    \label{proof-eq:reaches_def}
    \exists_{h \in \rhistories} \exists_{\agentfix \in \agentsbasis} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh').
\end{equation}

Then, negate this statement and repeatedly apply DeMorgan's Law for quantifiers:
\begin{align*}
    &\neg \exists_{h \in \rhistories} \exists_{\agentfix \in \agentsbasis} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \neg \exists_{\agentfix \in \agentsbasis} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \forall_{\agentfix \in \agentsbasis} \neg \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \forall_{\agentfix \in \agentsbasis} \exists_{h' \in \rsuffhistories}\ \agent(hh') \neq \agentfix(hh').
\end{align*}
The final statement is identical to the definition of never reaches, and thus, by the law of excluded middle, we conclude the proof. \qedhere
\end{dproof}

==> proofs/props/mb_agents_all_agents.tex <==
\begin{dproof}[\cref{prop:mbagents_is_allagents}]
The argument is actually quite straightforward, as for any agent $\agent^{\diamond} \in \allagents$, we can always consider the model-based learning rule defined over the singleton agent basis,
\begin{equation}
    \learnrule(h) = \argmax_{\agent \in \{\agent^{\diamond}\}} \valuef(\agent, \environment \mid h).
\end{equation}
Clearly, by necessity, the above learning rule will pick $\agent^{\diamond}$. Since $\agent^\diamond$ was chosen arbitrarily, we conclude that this construction holds for all agents. \qedhere
\end{dproof}

==> proofs/props/mb_agents_univbasis_all_agents.tex <==
\begin{dproof}[\cref{prop:univ_mbagents_is_allagents}]
The argument follows from the fact that every agent is optimal in at least one environment. To see this, note that the constant-zero reward function, $r(h) = 0$, ensures all agents are contained in the set of optimal agents. Then, pick an arbitrary agent $\agent^\diamond \in \allagents$. Note that by the first claim, each agent is optimal (for any choice of $\valuef$) in at least one environment. Call one of the environment's that $\agent^\diamond$ is optimal in $\environment^\diamond$. Then, the learning rule,
\begin{equation}
    \learnrule(h) = \argmax_{\agent \in \allagents} \valuef(\agent, \environment^\diamond \mid h),
\end{equation}
can be chosen to break $\argmax$ ties by always choosing $\agent^\diamond$. \qedhere
\end{dproof}

==> proofs/props/minimal_lim_size_implies_conv.tex <==
\begin{dproof}[\cref{prop:minimal_lim_size_implies_conv}]
Consider a fixed but arbitrary $(\agent,\env)$ pair such that $c_\infty(\agent,\env) \leq n$. Expanding the definition of $c_\infty$, this means that,
\begin{align*}
%
c_\infty(\agent,\env) &= \lim_{t \ra \infty} c_t(\agent,\env)\\
%
&= \lim_{t \ra \infty} \min \{k \in \mathbb{N} : \forall_{h \in \rhistories^{t:\infty}} \exists_{\agent_k \in \agents_k} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agent_k(hh')\}  \leq n.
\end{align*}
Therefore, there exists a choice of $k \leq n$ and set of bounded agents, $\agents_k$, such that% for all $t \geq 0$,
\[
\forall_{t \geq 0} \exists_{\agent_k \in \agents_k} \forall_{h \in \rhistories_{t:\infty}}\ \agent(h) = \agent_k(h).
\]
We can rewrite any realizable history $h$ in terms of the concatenation of three parts, $h = h^\diamond h^\circ h'$. 

\dnote{TODO}
\end{dproof}

==> proofs/props/notreaches_is_transitive.tex <==
\begin{dproof}[\cref{prop:never_reaches_is_transitive}]


% We proceed toward contradiction and suppose that both $\forall_{\agent^1 \in \agents^1}\ \agent^1 \notreaches \agents^2$ and $\forall_{\agent^2 \in \agents^2}\ \agent^2 \notreaches \agents^3$, but that $\neg \forall_{\agent^1 \in \agents^1}\ \agent^1 \notreaches \agents^3$. That is, rewriting the final assumption,
% \begin{align*}
% %
% \neg \forall_{\agent^1 \in \agents^1}\ \agent^1 \notreaches \agents^3 &= \exists_{\agent^1 \in \agents^1}\ \neg \agent^1 \notreaches \agents^3, \\
% %
% &= \exists_{\agent^1 \in \agents^1}\ \agent^1 \reaches \agents^3.
% \end{align*}
% where the first equality holds by DeMorgan's law for quantifiers, and the second equality holds by \cref{prop:eventually_xor_never_reaches}.

% % 
% Denote the $\agent^1 \in \agents^1$ for which $\agent^1 \canreach \agents^3$ as $\bar{\agent}^1$. By definition of can reach, we know that
% \[
% \exists_{h \in \rhistories} \exists_{\agent^3 \in \agents^3} \forall_{h' \in \rsuffhistories}\ \bar{\agent}^1(hh') = \agent^3(hh').
% \]


\end{dproof}

==> proofs/props/other_basis_not_crl.tex <==
\begin{dproof}[\cref{prop:other_basis_not_crl}]
Recall that a tuple $(\env, \valuef, \agents, \agentsbasis)$ is CRL just when all of the optimal agents $\agents^*$ do not reach the basis.
%
Then, the result holds as a straightforward consequence of two facts.
%
% First.
First, we can always construct a new basis containing all of the optimal agents, $\agentsbasis^\circ = \agentsbasis \cup \agents^*$.
%
% Second.
Second, by \cref{prop:agent_in_set_reaches_set}, we know that every element $\agentbasis^\circ \in \agentsbasis^\circ$ will always reach the basis, $\agentbasis^\circ \alwaysreaches \agentsbasis^\circ$. Therefore, in the tuple $(\env, \valuef, \agents, \agentsbasis^\circ)$, each of the optimal agents will reach the basis, and therefore this is not an instance of CRL. \qedhere
\end{dproof}

==> proofs/props/superset_generates.tex <==
\begin{dproof}[\cref{prop:superset_generates}]
The result follows as a natural consequence of the definition of generates. Recall that $\agentsbasis^1 \unifgenerates \agents$ just when,
\begin{align}
    \label{eq:proof_eq_generates_def}
    &\exists_{\learnrules^1 \subseteq \alllearnrules}\ \agentsbasis^1 \unifgenerates_{\learnrules^1} \agents \\
    %
    %
    \equiv\ &\exists_{\learnrules^1 \subseteq \alllearnrules}\ \exists_{\learnrule^1 \in \learnrules^1} \forall_{h \in \rhistories}\ \agent(h) = \agentbasis^{\learnrule^1(h)}(h),
\end{align}
where again $\agentbasis^{\learnrule^1(h)} \in \agentsbasis^1$ is the base agent chosen by $\learnrule^1(h)$. We use superscripts $\learnrules^1$ and $\learnrule^1$ to signify that $\learnrule^1$ is defined relative to $\agentsbasis^1$, that is,  $\learnrule^1 : \histories \ra \agentsbasis^1 \in \learnrules^1$.

But, since $\agentsbasis^1 \subseteq \agentsbasis^2$, we can define $\learnrules^2 = \learnrules^1$ and ensure that $\agentsbasis^2 \unifgenerates_{\learnrules^2} \agents$, since the agent basis $\agentsbasis^1$ was already sufficient to generate $\agents$.  Therefore, we conclude that $\agentsbasis^2 \unifgenerates \agents$. \qedhere
\end{dproof}

==> proofs/thm-agent_gen_undecidable.tex <==
\begin{dproof}[\cref{thm:agent_gen_undecidable}]
We proceed as is typical of such results by reducing \textsc{AgentsGenerate} from the Halting Problem.

In particular, let $m$ be a fixed but arbitrary Turing Machine, and $w$ be a fixed but arbitrary input to be given to machine $m$. Then, \textsc{Halt} defines the decision problem that outputs True iff $m$ halts on input $w$.

We construct an oracle for \textsc{AgentsGenerate} that can decide \textsc{Halt} as follows. Let $(\actions, \observations)$ be an interface where the observation space is comprised of all configurations of machine $m$. Then, we consider a deterministic environment $\env$ that simply produces the next configuration of $m$ when run on input $w$, based on the current tape contents, the state of $m$, and the location of the tape head. Note that all three of these elements are contained in a Turing Machine's configuration. Now, let the action space $\actions$ consist of two actions, $\{a_{\text{no-op}}, a_{\mr{halt}}\}$. On execution of $a_{\text{no-op}}$ no-op, the environment moves to the next configuration. On execution of $a_{\mr{halt}}$, the machine halts. That is, we restrict ourselves to the singleton agent set, $\agents$, containing the agent that outputs $a_{\mr{halt}}$ directly following the machine halting, and $a_{\text{no-op}}$ otherwise.

Using these ingredients, we take any instance of \textsc{Halt}, $(m,w)$, and build the agent set: $\agentsbasis^1 = \{a_{\text{no-op}}\}$. We make one query to our \textsc{AgentsGenerate} oracle, and ask: $\agentsbasis^1 \generates \agents$. If it is True, then the single agent in $\agents$ never emits the $a_{\text{halt}}$ action, and thus, $m$ does not halt on $w$. If it is False, then there are realizable histories in $\env$ in which $m$ halts on $w$. We thus use the oracle's response directly to decide the given instance of \textsc{Halt}. \qedhere
\end{dproof}

==> proofs/thm-agent_reaches_undecidable.tex <==
\begin{dproof}[\cref{thm:agent_reaches_undecidable}]
We again proceed by reducing \textsc{AgentReaches} from the Halting Problem.

In particular, let $m$ be a fixed but arbitrary Turing Machine, and $w$ be a fixed but arbitrary input to be given to machine $m$. Then, \textsc{Halt} defines the decision problem that outputs True iff $m$ halts on input $w$.

We construct an oracle for \textsc{AgentReaches} that can decide \textsc{Halt} as follows. Consider the same observation space used in the proof of \cref{thm:agent_gen_undecidable}: Let $\observations$ be comprised of all configurations of machine $m$. Then, sequences of observations are simply evolution of different Turing Machines processing possible inputs. We consider an action space, $\actions = \{a_{\mr{halted}}, a_{\mr{not-yet}}\}$, where agents simply report whether the history so far contains a halting configuration. 

Then, we consider a deterministic environment $\env$ that simply produces the next configuration of $m$ when run on input $w$, based on the current tape contents, the state of $m$, and the location of the tape head. Note again that all three of these elements are contained in a Turing Machine's configuration.

Using these ingredients, we take any instance of \textsc{Halt}, $(m,w)$, and build the singleton agent set $\agentsbasis$ containing only the agent $\agent_{\mr{halted}} : h \mapsto a_{\mr{halted}}$ that always reports the machine as having halted. We then consider whether the agent that outputs $a_{\mr{not-yet}}$ indefinitely until $m$ reports halting, at which point the agent switches to $a_{\mr{halted}}$.

We make one query to our \textsc{AgentReaches} oracle, and ask: $\agent \reaches \agentsbasis$. If it is True, then the branching agent eventually becomes equivalent to $\agent_{\mr{halted}}$ in that they both indefinitely output $ a_{\mr{halted}}$ on at least one realizable history. Since $\env$ is deterministic, we know this equivalence holds across all histories. If the query reports False, then there is no future in $\env$ in which $m$ halts on $w$, otherwise the agent would become equivalent to $\agent_{\mr{halted}}$. We thus use the oracle's response directly to decide the given instance of \textsc{Halt}. \qedhere
\end{dproof}

==> proofs/thm-mb_plan_inf_often.tex <==
\begin{dproof}[\cref{thm:crl_mb_plan_inf_often}]
% Strategy.
We proceed toward contradiction and assume that there is a CRL problem in which an optimal model-based agent $\agent^*$ only replans finitely many times.

% Proof.
That is, we assume that there is an optimal model-based agent, $\agent^* \in \agents^*$ whose corresponding learning rule $\learnrule$ satisfies the following: $\exists_{h \in \rhistories} \forall_{h' \in \rsuffhistories}$ such that,
\begin{equation*}
    \underbrace{\argmax_{\agent \in \agentsbasis} \valuef(\agent, \hat{\env} \mid h)}_{\learnrule(h)} = \underbrace{\argmax_{\agent \in \agentsbasis} \valuef(\agent, \hat{\env} \mid hh')}_{\learnrule(hh')}.
\end{equation*}

Then, consider the behavior of $\agent^*$ at some realizable history $h$. By the above equivalence, we know that for \textit{every} realizable suffix $h'$ that might follow $h$, the agent will produce the same behavior, $\agent \in \agentsfix$, output from
\begin{equation}
    \argmax_{\agent \in \agentsbasis} \valuef(\agent, \hat{\env} \mid h).
\end{equation}
Therefore, it follows that $\agent^* \reaches \agentsbasis$: there exists a realizable history under which $\agent^*$ will produce the same behavior as an element from $\agentsbasis$ on all futures. However, recall that by assumption we are in a CRL problem, meaning all optimal agents must never reach $\agentsbasis$.

We have reached a contradiction, and thus conclude the proof. \qedhere
\end{dproof}

==> proofs/thm-reaches_insight.tex <==
\begin{dproof}[\cref{thm:reaches_insight}]
The proof of the first property is straightforward, as sometimes and never reaches are simply logical negations of one another.

That is, recall the definition of \textit{sometimes reaches} for a fixed but arbitrary $(\agent, \agentsfix)$ pair:
\begin{equation}
    \exists_{h \in \rhistories} \exists_{\agentfix \in \agentsfix} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh').
\end{equation}

Then, negate this statement and repeatedly apply DeMorgan's Law for quantifiers:
\begin{align*}
    &\neg \exists_{h \in \rhistories} \exists_{\agentfix \in \agentsfix} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \neg \exists_{\agentfix \in \agentsfix} \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \forall_{\agentfix \in \agentsfix} \neg \forall_{h' \in \rsuffhistories}\ \agent(hh') = \agentfix(hh'),\\
    %
    %
    &\equiv \forall_{h \in \rhistories} \forall_{\agentfix \in \agentsfix} \exists_{h' \in \rsuffhistories}\ \agent(hh') \neq \agentfix(hh').
\end{align*}
The final statement is identical to that given by the agent \textit{never} reaches operator, and thus, by the law of excluded middle, we conclude. \checkmark \\

% Second property.
The second property notes that, for any $(\agents, \env)$ pair, we can identify a basis such that $\agents$ is split into two non-empty sets: those agents that \textit{sometimes reach} the basis, and those that \textit{never reach} the basis.

To show this, consider a fixed but arbitrary $(\agents, \env)$ with $|\agents| \geq 2$. Pick an agent in $\agents$, call it $\agent^\circ$, and build a basis, $\agentsbasis^\circ = \{\agent^\circ\}$. Clearly, by \cref{lem:agent_in_set_reaches_set}, $\agent^\circ \reaches \agentsbasis^\circ$. Now, pick another agent in $\agents$, call it $\agent^\diamond$. By definition, we know there exists at least one history, $h$, such that $\agent^\circ(h) \neq \agent^\diamond(h)$. Let $\env$ be an environment that places non-zero probability mass on $h$ when interacting with both $\agent^\circ$ or $\agent^\diamond$. Then, clearly 

\qedhere
\end{dproof}

==> proofs/thm-reaches_transitive.tex <==
\begin{dproof}[\cref{thm:reaches_transitive}]

We construct two counterexamples, one for each of ``sometimes reaches" ($\reaches)$ and ``never reaches'' ($\notreaches$).


% Sometimes.
%
\paragraph{Counterexample: Sometimes Reaches.} To do so, we begin with a tuple $(\env, \agents^1, \agents^2, \agents^3)$ such that both
\[
\forall_{\agents^1 \in \agents^1}\ \agent^1 \reaches \agents^1,\hspace{8mm} \forall_{\agents^2 \in \agents^2}\ \agent^2 \reaches \agents^2.
\]
We will show that there is an agent, $\overline{\agent}^1 \in \agents^1$, such that $\overline{\agent}^1 \notreaches \agents^3$, thus illustrating that sometimes reaches is not transitive. The basic idea is that sometimes reaches only requires an agent stop its search on \textit{one} realizable history. So, $\agent^1 \reaches \agents^2$ might happen on some history $h$, but each $\agent^2 \in \agents^2$ might only reach $\agents^3$ on an entirely different history. As a result, reaching $\agents^2$ is enough to ensure the agent also reaches $\agents^3$.


% Agent set details.
In more detail, the agent sets of the counterexample are as follows. Let $\actions = \{a_1, a_2\}$ and $\observations = \{o_1, o_2\}$. Let $\agents^2$ be all agents that, after ten timesteps, always take $a_2$. $\overline{\agent}^1$ is simple: it always takes $a_1$, except on one realizable history, $h^\circ$, (and all of this histories realizable successors), where it switches to taking $a_2$ after ten timesteps. Clearly $\overline{\agent^1} \reaches \agents^2$, since after ten timesteps, we know there will be some $\agent^2$ such that $\overline{\agent}^1(h^\circ h') = \agent^2(h^\circ h')$ for all realizable history suffixes $h'$. Now, by assumption, we know that $\agent^2 \reaches \agents^3$. This ensures there is a \textit{single} realizable history $h$ such that there is an $\agent^3$ where $\agent^2(hh') = \agent^3(hh')$ for any realizable suffix $h'$. To finish the counterexample, we simply note that this realizable $h$ can be different from $h^\circ$ and all of its successors. For example, $h^\circ$ might be the history containing only $o_1$ for the first ten timesteps, while $h$ could be the history containing only $o_2$ for the first ten timesteps. Thus, this $\agent^1$ never reaches $\agents^3$, and we conclude the counterexample. \checkmark \\


\paragraph{Counterexample: Never Reaches.} The instance for never reaches is simple: Let $\actions = \{a_1, a_2, a_3\}$, $\agents^1 = \agents^3$. Suppose all agents in $\agents^1$ (and thus $\agents^3$) only choose actions $a_1$ and $a_3$. Let $\agents^2$ be a singleton, $\agents^2 = \{\agent^2\}$ such that $\agent^2 : h \mapsto a_2$. Clearly, every $\agent^1 \in \agents^1$ will never reach $\agents^2$, since none of them ever choose $a_2$. Similarly, $\agent^2$ will never reach $\agents^3$, since no agents in $\agents^3$ choose $a_2$. However, by \cref{prop:agent_in_set_reaches_set} and the assumption that $\agents^1 = \agents^3$, we know $\forall_{\agent^1 \in \agents^1}\ \agent^1 \alwaysreaches \agents^3$. This directly violates transitivity. \checkmark

%suppose that every agent $\agent^2 \in \agents^2$ does \textit{not} reach $\agents^3$ on $h^\circ$ or any of its successors. Instead, 

This completes the argument for all three cases, and we conclude. \qedhere

\end{dproof}
